Trim My View: An LLM-Based Code Query System for Module Retrieval in Robotic Firmware

The software compilation process has a tendency to obscure the original design of the system and makes it difficult both to identify individual components and discern their purpose simply by examining the resulting binary code. Although decompilation techniques attempt to recover higher-level source code from the machine code in question, they are not fully able to restore the semantics of the original functions. Furthermore, binaries are often stripped of metadata, and this makes it challenging to reverse engineer complex binary software. In this paper we show how a combination of binary decomposition techniques, decompilation passes, and LLM-powered function summarization can be used to build an economical engine to identify modules in stripped binaries and associate them with high-level natural language descriptions. We instantiated this technique with three underlying open-source LLMs -- CodeQwen, DeepSeek-Coder and CodeStral -- and measured its effectiveness in identifying modules in robotics firmware. This experimental evaluation involved 467 modules from four devices from the ArduPilot software suite, and showed that CodeStral, the best-performing backend LLM, achieves an average F1-score of 0.68 with an online running time of just a handful of seconds.

==> src/shunt/intro.tex <==
\section{Introduction}
\label{intro}

\begin{figure*}
\centering
\includegraphics[width=.7\textwidth]{images/figure1-1.pdf}
\caption{The Workflow of the ChatCPS system. A) ChatCPS decomposes the binary firmware into its modules. B) Shows the decompilation process. $F_n$ indicates binary functions, while $F_n^*$ indicates the corresponding decompiled functions. C) ChatCPS summarizes each function in a module using three open-source LLMs (CodeQwen, CodeStral, DeepSeek-Coder) and D) categorizes modules based on function descriptions. }
\label{fig:chatcps-workflow}
\end{figure*}

In programming, particularly in languages like C and C++, a module refers to a self-contained unit of source code designed to achieve a specific functionality. This modular approach allows developers to encapsulate related functions, data structures, and operations within a single unit, promoting code reusability and maintainability. Functions within a module are organized together to serve a specific functionality. In areas such as robotic vehicles and embedded systems, there are specialized modules designed to handle communication protocols such as Serial Peripheral Interface (SPI) and Universal Asynchronous Receiver/Transmitter (UART), among others. Identifying and searching for specific functionalities in these complex software systems, which usually contain a large number of functions, is essential for understanding the software structure.

Due to concerns about patent infringement, the source code for software, especially the embedded system firmware is often not readily available; instead, only the compiled version, known as a binary, is accessible. During compilation, meta-information about code, such as type information, is lost. Decompilation, the process of transforming binary programs back into a higher-level, more human-readable form of source code, is unable to fully recover the semantic details of the original code~\cite{cao2024evaluating}. Furthermore, binary programs are typically stripped of function and variable names, which significantly complicates understanding of the code.

Recently, researchers have begun to leverage LLMs to enhance code semantic understanding, with applications ranging from binary code summarization~\cite{jin2023binary, song2024bin2summary} and source-to-binary matching~\cite{jiang2024binaryai} to function identification~\cite{chen2024foc}. 

There are several research studies evaluating LLMs for function summarization tasks~\cite{jin2023binary, song2024bin2summary, al2023extending, mastropaolo2024evaluating, ahmed2022few}, but two main issues persist with the current studies.

First, function summarization, while useful for gaining a broad understanding of what a function does, may not be entirely sufficient for specific needs, especially in fields like reverse engineering, where detailed knowledge of particular functionalities is essential. In malware analysis, reverse engineers frequently target distinct behaviors that signal malicious activities, such as keylogging, unauthorized network communications, or manipulations of system processes. These essential functionalities are often deeply embedded in the code and are triggered under specific conditions, making them challenging to detect through general function summarization alone. This complexity requires a more detailed and focused analysis approach, surpassing what broad summarization techniques generally provide. Moreover, analyzing individual function summaries cannot reveal the underlying architecture of software, which is essential for comprehensive software analysis.

Second, there is extensive research and evaluation focused on well-known LLMs like GPTX~\cite{achiam2023gpt}, Copilot\footnote{\url{https://copilot.github.com/}}, Gemini~\cite{anil2023gemini}, etc. Meanwhile, open-source LLMs~\cite{bai2023qwen, zhu2024deepseek} often receive less attention, leaving their potential in this field under-explored. In addition, the high costs associated with commercial models make these resources difficult for many individual researchers to access. For instance, BinSum\cite{jin2023binary} incurred a \$11,000 expense to use GPT-4 for their evaluation.

To address these challenges, we designed an LLM-based code query system to retrieve module categories in stripped binary firmware by leveraging three open-source LLMs: CodeQwen~\cite{hui2024qwen2}, DeepSeek-Coder~\cite{zhu2024deepseek}, and CodeStral~\cite{chaplot2023albert}. We selected three mid-sized large language models (LLMs) from the BigCodeBench leaderboard~\cite{bigcode2023leaderboard}. These models were chosen based on their performance on the BigCodebench~\cite{zhuo2024bigcodebench} tasks.

To design the system, we first break down the binary into its modular components, by implementing the modified version of the BCD\cite{karande2018bcd} algorithm. Then, we utilize LLMs to summarize the functionality of each decompiled function in the module. Finally, we categorize modules based on the function descriptions. In this way, users can search and aim for a specific module category.  In this paper, we define four module categories encoded by CPS expert knowledge including data transfer, navigation, controller, and safety check. We describe each category in detail in Section~\ref{sec:chatcps:module_ret}.

Moreover, since these module categories are built on top of function summaries, we develop a source code parser to evaluate their quality. This parser extracts the source code function bodies and then normalizes the functions by removing comments, variables, and function names.

Designing this system offers multiple benefits. First, it streamlines the reverse engineering process, making it more accessible. Second, it enables users to efficiently navigate through various functionalities within the codebase. Moreover, the module categorization system enhances the understanding of the binary program's underlying structure and framework. Additionally, it creates a foundation for more specific queries within each module. For instance, some robotic firmware frequently uses known mathematical algorithms such as the Kalman Filter~\cite{kalman1960new} and Proportional, Integral, Derivative (PID)~\cite{visioli2006practical} controller algorithms. These types of algorithms can be found in navigation and controller modules. Moreover, after recovering modules that implement communication protocols (e.g., UART, MAVLink), users can run specific queries about the structure of the messages being sent and received, including headers, payloads, and trailers.

Extensive research has been conducted on well-known LLMs like GPT-X~\cite{achiam2023gpt,Brown2020LanguageMA}, Claude~\cite{anthropic_claude}, Copilot~\cite{github_copilot}, etc., whose API services are often costly. Given that complex software typically comprises a large number of functions, the expense of running such queries can be prohibitive for individual researchers. Therefore, in this study, we opt for an evaluation using three open-source LLMs to ensure practicality and accessibility. You can find detailed explanations of each evaluation phase of our system in Sections~\ref{sec:exprimental_setup} and~\ref{sec:exper_result}.

To our knowledge, this is the first instance of a code query-based system that utilizes LLMs to retrieve specific functionalities within stripped binaries. Here is a list of our contributions.

\begin{itemize}
  \item We implement a new variant of the BCD algorithm adjusted for our needs and evaluate its effectiveness in decomposing robotic firmware into modular components within cyber-physical systems. In addition, we will make the source code publicly available to facilitate further research and development in this area.
  \item We evaluate the effectiveness of three open-source LLMs, DeepSeek-Coder, CodeQwen, and CodeStral, in summarizing decompiled functions within modules for stripped firmware and develop a method to parse and normalize source code for evaluating the quality of these summaries.
  \item We have developed a code-based query system that defines and retrieves various module categories using summaries of functions generated by LLMs.
  \item We establish the ground truth to define the categories for 467 modules across four devices in the ArduPilot~\cite{ardupilot_dataset} dataset, including QuadCopter, HeliCopter, Rover, and Submarine.
\end{itemize}


%Since some categories are common between robotic vehicles, we choose five categories including data transfer, navigation, controller, safety check, configuration and calibration. We also consider one category \textit{other}, if it does not fit in any of the aforementioned categories. 
The rest of the paper is organized as follows: Section~\ref{sec:related} provides a summary of existing similar techniques. In Section~\ref{sec:chatcps}, we propose the architecture and design of our system, ChatCPS. The implementation details and results of our experimental evaluation are presented in Sections~\ref{sec:exprimental_setup} and~\ref{sec:exper_result}, respectively. Lastly, we discuss the limitations of our approach and potential future work in Sections~\ref{sec:limitations} and~\ref{sec:future_work}, respectively.


